Pattern Tree: Enhancing Efficiency in Quantum Circuit Optimization Based on Pattern-matching

Quantum circuit optimization is essential for improving the performance of quantum algorithms, particularly on Noisy Intermediate-Scale Quantum (NISQ) devices with limited qubit connectivity and high error rates. Pattern matching has proven to be an effective technique for identifying and optimizing subcircuits by replacing them with functionally equivalent, efficient versions, including reducing circuit depth and facilitating platform portability. However, existing approaches face challenges in handling large-scale circuits and numerous transformation rules, often leading to redundant matches and increased compilation time. In this study, we propose a novel framework for quantum circuit optimization based on pattern matching to enhance its efficiency. Observing redundancy in applying existing transformation rules, our method employs a pattern tree structure to organize these rules, reducing redundant operations during the execution of the pattern-matching algorithm and improving matching efficiency. We design and implement a compilation framework to demonstrate the practicality of the pattern tree approach. Experimental results show that pattern-tree-based pattern matching can reduce execution time by an average of 20% on a well-accepted benchmark set. Furthermore, we analyze how to build a pattern tree to maximize the optimization of compilation time. The evaluation results demonstrate that our approach has the potential to optimize compilation time by 90%.

==> assests/alg-sch-bak.tex <==
\IncMargin{1em}
\begin{algorithm}
\Input{Input DAG $\mathcal{G}$, a given transformation rule $r$}
\Output{Rewritten DAG $\mathcal{G}'$}
\Fn{\Scheduler{$\mathcal{G},r$}}{
    \Context$\leftarrow$ \PM{$\mathcal{G}$, $r$}\;
    \If{\Context}{
        \If{$r$.\Succ}{
            $r'\leftarrow$ $r$.\Succ\;
            \newC$\leftarrow$ \PM{$\mathcal{G}$, $r$}\;
            \While{\newC $\mathrm{or}$ $r$.\Sibling}{
                \uIf{\newC}{
                    \Context$\leftarrow$ \newC, $r\leftarrow r'$\;
                    \uIf{$r$.\Succ}{
                        $r\leftarrow$ $r$.\Succ\tcp*[r]{Parent relation}
                    }
                    \Else{
                        break\;
                    }
                }
                \ElseIf{$r$.\Sibling}{
                    $r\leftarrow$ $r$.\Sibling\tcp*[r]{Sibling relation}
                }
            }
        }
        \If{\IsOpt{$r$}}{
            \Return{\Rewrite{$\mathcal{G}$,$r$,\Context}}\;
        }
    }
}
\caption{Pattern-matching scheduler}
\label{alg:sche}
\end{algorithm}
\DecMargin{1em}

==> assests/fig-pt-bak.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.46\textwidth]{assests/fig/pt.png}
    \caption{PTree}
    \label{fig:pt}
\end{figure}

==> assests/fig-rt.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.4\textwidth]{assests/fig/rt.png}
    \caption{RTree}
    \label{fig:rt}
\end{figure}

==> assests/fig-rz-com.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.35\textwidth]{assests/fig/rz-1.png}
    \caption{Commutation rules for $R_z$ gate}
    \label{fig:rz-com}
\end{figure}

==> assests/tbl-pt.tex <==
\begin{table}[ht]\tiny
    \centering
    \begin{tabular}{|c|c|c|ccc|}
        \hline
        Circuit & Orig. & q & \makecell{Time(ms) \\ (w/o p.t.)} & \makecell{Time(ms) \\ (w/ sp=18)} & Speedup \\
        \hline
        adder\_8         & 900 & 24  & 180142.926   & 24845.277 & 7.25 \\
        barenco\_tof\_3  & 58  & 5   &  3065.364   & 1006.338  & 3.04 \\
        barenco\_tof\_4  & 114 & 7   &  7045.197    & 1556.835  & 4.52 \\
        barenco\_tof\_5  & 170 & 9   &  12075.853    & 2253.362  & 5.35 \\
        barenco\_tof\_10 & 450 & 19  &  52195.616   & 7748.472  & 6.73 \\
        csla\_mux\_3     & 170 & 15  &  13856.069   & 2422.842  & 5.71 \\
        csum\_mux\_9     & 420 & 30  &  49954.320   & 7823.455  & 6.38\\
        mod5\_4          & 63  & 5   &  3796.818    & 1213.332  & 3.12 \\
        mod\_mult\_55    & 119 & 9   &  7627.371    & 2069.635  & 3.68\\
        mod\_red\_21     & 278 & 11  &  23954.040   & 4048.827  & 5.91\\
        qcla\_adder\_10  & 521 & 36  &  72786.406   & 10094.265 & 7.21\\
        qcla\_com\_7     & 443 & 24  &  52719.437   & 8118.469  & 6.49\\
        qcla\_mod\_7     & 884 & 26  &  182023.710  & 25062.336 & 7.26\\
        rc\_adder\_6     & 200 & 14  &  17549.561   & 3886.253  & 4.51\\
        tof\_3           & 45  & 5   &  2180.890    & 893.454   & 2.44 \\
        tof\_4           & 75  & 7   &  3898.971    & 1129.918  & 3.45\\
        tof\_5           & 105 & 9   &  5865.516    & 1404.586  & 4.17\\
        tof\_10          & 255 & 19  &  19702.195   & 3311.221  & 5.95\\
        vbe\_adder\_3    & 150 & 10  &  11335.113   & 2152.018  & 5.26\\
        gf2\textasciicircum4\_mult     & 225 & 12  & 20831.580  & 3325.705  & 6.26\\
        gf2\textasciicircum5\_mult     & 347 & 15  & 40746.416  & 5824.115  & 6.99\\
        gf2\textasciicircum6\_mult     & 495 & 18  & 71694.096  & 9786.297  & 7.32 \\
        gf2\textasciicircum7\_mult     & 669 & 21  & 119479.888 & 15819.492 & 7.55\\
        gf2\textasciicircum8\_mult     & 883 & 24  & 198320.288 & 25777.268 & 7.69 \\
        gf2\textasciicircum9\_mult     & 1095 & 27 & 287493.256 & 36835.225 & 7.80\\
        gf2\textasciicircum10\_mult    & 1347 & 30 & 420873.118 & 53845.641 & 7.81\\
        \hline
        \multicolumn{5}{|c|}{\kd{Mean Acc. Rate}} & 5.76  \\
        \hline
    \end{tabular}
    \caption{The optimization effect taken by the pattern-tree-based pattern library}
    \label{tbl:opt-time}
\end{table}


==> sections/ack.tex <==
\section*{Acknowledgement}
{
This work was partly supported by the grants of the Innovation Program for Quantum Science and Technology (No. 2021ZD0302300), the National Natural Science Foundation of China (No. 62272434), the Fundamental Research Funds for the Central Universities (No. WK2060000018).
}

==> sections/eval-bak.tex <==
\section{Evaluation}
\label{sec:eval}
In this section, we demonstrate the effects of pattern tree in reducing the size of pattern library, and evaluate its optimization effects on the execution time of pattern matching algorithm. 
% and evaluate its effects on accelerating pattern matching algorithm. 

This section is structured as follows: First, we provide the experimental setup, including benchmarks, experiment platform, and the transformation rules used for pattern matching.
Then, we present the optimization effect of pattern tree on the number of transformation rules in the pattern library. 
%Finally, we will demonstrate the comparison of the optimization effect of optimized pattern library with the original pattern library in terms of quantum circuit optimization effects.
Finally, we demonstrate the comparison of the execution time of optimized pattern library with the original pattern library in terms of pattern matching algorithm.


\subsection{Experiment setup}

Our framework is evaluated by using 12th Gen Intel(R) Core(TM) i9-12900K and is based on the pattern-matching framework \textsc{QCiR}\cite{chen2022qcir}. 
% We use \textsc{QCiR}'s pattern description format to express transformation rules. 
We generate transformation rules by Quartz\cite{xu2022quartz} and then convert them to \textsc{QCiR}'s format. 
% Since we are the first to consider optimizing pattern-matching algorithm, there are no compiler for us to compare our optimization effect. 

We use the benchmark suite of 26 circuits used by prior work\cite{nam2018automated, xu2022quartz,iten2022exact}. All \kn{R}$_z$ gates in the benchmarks are initially converted to \kn{T} and \kn{T}$^\dagger$ gates for matching, prior to optimization.

\input{assests/tbl-red}
\vspace{-2em}

\subsection{Reduction in the number of rules}

We choose to use Quartz\cite{xu2022quartz} to automatically generate transformation rules. The gate set we use is $\{$\kn{T},\kn{T}$^\dagger$, \kn{X}, \kn{H} and \kn{CNOT}$\}$. In order to express pattern relations in the pattern library, an extra file is added to express the edges on the pattern tree. We use the fingerprint generated by Quartz as the unique id of transformation rule.

Table.\ref{tbl:red} shows the reduction in the number of rules by pattern tree.
The parameter $n$ and $q$ are used to specify the transformation rules are at most $n$ gates and $q$ qubits. Details can be found in \cite{xu2022quartz}. The Orig. column is the number of rules generated given $n$ and $q$. The size of pattern tree means how many rules can be combined with other rules to simplify their matching procedure. As we claimed in the Sec.\ref{sec:des}, not all rules can be added to the pattern tree to speed up the pattern matching algorithm. Only rules have one of two relations will be added to pattern tree together to simplify matching. The branches column specifies how many rules we packed the rules on pattern tree into.
For example, for $n=3$ and $q=4$, 91 rules out of 221 rules are added to pattern tree, and 21 out of 91 rules are used as start point of their respective subtree. In other words, 91 rules are compressed into 21 new rules.
On the selection of the rules as start point, we use original rules instead of the special rules corresponding to the blank node as possible.

% In order to implement pattern tree, we use an unique id to represent each transformation rule, and add an extra file including multiple parent-child relations to represent relations between nodes. 
% For implementation, we delete the blank nodes which are not common ancestor of multiple orange nodes, as shown in the upper and lower box of Fig.\ref{fig:tree}. Since we don't take null string as a node, in fact the rules will be optimized into a pattern forest instead of pattern tree.
% Since some rules cannot be better expressed by our relation tree, we finally generate a rule tree to compress 355 rules in pattern library into 16 rules by the representative set from Quartz.

\subsection{Experiment results}

\input{assests/tbl-opt}

Table.\ref{tbl:opt} compares the execution time of optimized pattern-matching algorithm with non-optimized algorithm. Here we use the pattern library by setting $n=3$ and $q=5$.
The optimization rate for each circuit basically fluctuates around 20\%. The average optimization rate for compilation time is 18\%. 
Since the pattern matching algorithm matches patterns on input circuit one by one and there is not much difference in size between source patterns of transformation rules, it's natural that the execution time of pattern matching algorithm is linearly related to the number of patterns. 
It is reasonable to speculate that the reduction in the number of transformation rules contributed to the execution time.


==> sections/moti.tex <==
\section{Motivation}
\label{sec:motv}
This section presents the motivation examples 

Fig.\ref{fig:motv-a} illustrates two transformation rules. Consider an input circuit with one qubit and three quantum gates. Assume that the matching algorithm matches rules A and B sequentially. Initially, matching rule A fails, followed by a successful match of rule B. The failure to match rule A causes the loss of all matching context, forcing the algorithm to re-check the first two gates of the input circuit when matching rule B. This increases the cost of the matching process and affects the algorithm's performance.

Fig.\ref{fig:motv-b} shows a different situation where the source pattern of rule C is a prefix of the source pattern of rule D. As a result, the match for rule D may include a match for rule C, potentially leading to unnecessary matching. However, if we simply remove rule C, we may lose some optimization opportunities.

%Fig.\ref{fig:motv-b} presents a different scenario. Rule C's source pattern is a prefix of rule D's source pattern. As a result, since the match for rule D includes the match for rule C, this potentially leads to unnecessary matching processes. However, if we were to simply remove rule C, we might lose some optimization opportunities.

An intuitive idea is to introduce common prefixes during the pattern matching process. When the common prefix of multiple rules' source patterns is specified, the compiler can revert to the prefix pattern to start matching other rules after a failed match, thus reducing the overhead. However, this approach has not been explored in existing work. In some papers, a template format is used \cite{iten2022exact}, which describes an identity circuit. The compiler matches the largest sub-circuit it can, and if the size of the largest sub-circuit exceeds the remaining part of the template, it replaces the matched circuit with the remaining part, thereby reducing the circuit's size. The template only addresses the second situation mentioned above.

%Some works consider the relationships between transformation rules, but do not provide solutions. In quantum circuit pattern matching, when using templates rather than transformation rules\cite{iten2022exact}, although templates can solve the second case, they cannot solve the first case. In the work of Nam \etal\cite{nam2018automated}, based on the influence of different transformation rules on circuits, subroutines are proposed to apply transformation rules in a specific order to maximize optimization effects. In the work of Xu \etal\cite{xu2022quartz}, they noticed redundancy in the process of generating rules, while what we point out here is redundancy existing in matching. Instead of deleting useless rules, We focus on efficiently utilizing all potentially useful rules.

Implementing common prefixes also poses challenges. In the two sets of rules we demonstrated, we observe that the common prefixes in both sets cannot be optimized. How to add unoptimized common prefixes to the pattern library also presents a challenge.


==> sections/related-bak.tex <==
\section{Related Work}
\label{sec:rel}
The optimization of quantum circuit is one of the key challenges for quantum computation in the NISQ era. 
Several optimization techniques have been proposed and developed.
Pattern matching is a promising technique for addressing this challenge. It has been recognized in many applications, such as classical compilation\cite{lattner2021mlir, espindola2023source}, subgraph matching\cite{zhang2024comprehensive}.
Several quantum compilation framework have adopted it as peephole optimization, such as Qiskit\cite{qiskit2024}, t|ket$\rangle$\cite{sivarajah2021tket}.

% Recent works on pattern matching of quantum circuits tend to focus on two directions.
Some pattern-matching work focus on improving the execution efficiency of pattern-matching algorithm.
Iten \etal\cite{iten2022exact} propose an exact quantum circuit pattern matching algorithm to provably discover all maximal matches. 
Rahman \etal\cite{rahman2014algorithm} introduce a heuristic pattern matching algorithm.

The other work focus on improving the optimization effect. Among them, the expansion of pattern library is one of the major research directions.
Nam \etal\cite{nam2018automated} present several transformation rules tailored to \{\kn{H}, \kn{X}, \kn{R}$_z$, \kn{CNOT}\} gate set for optimizing quantum circuits. Transformation rules for high-level modules are also studied. Maslov \etal\cite{maslov2016advantages} consider replacing multi-control Toffoli gates with simpler relative-phase versions.
Observing this trend, automatic generation of transformation rules is raised to reduce manual efforts.
Quanto\cite{pointing2021optimizing} is the first quantum circuit optimizer that automatically generates circuit identities to reduce manual efforts.
After that, Xu \etal\cite{xu2022quartz} developed a quantum circuit superoptimizer Quartz, which can not only automatically generate but verify transformation rules.

Also, the implementation of the pattern library is also a research direction.
Chen \etal\cite{chen2022qcir} design QCiR framework with designing a new pattern description format to support scalability for future transformation rules.

